Task Parallel Incomplete Cholesky Factorization using 2D Partitioned-Block Layout

We introduce a task-parallel algorithm for sparse incomplete Cholesky factorization that utilizes a 2D sparse partitioned-block layout of a matrix. Our factorization algorithm follows the idea of algorithms-by-blocks by using the block layout. The algorithm-by-blocks approach induces a task graph for the factorization. These tasks are inter-related to each other through their data dependences in the factorization algorithm. To process the tasks on various manycore architectures in a portable manner, we also present a portable tasking API that incorporates different tasking backends and device-specific features using an open-source framework for manycore platforms i.e., Kokkos. A performance evaluation is presented on both Intel Sandybridge and Xeon Phi platforms for matrices from the University of Florida sparse matrix collection to illustrate merits of the proposed task-based factorization. Experimental results demonstrate that our task-parallel implementation delivers about 26.6x speedup (geometric mean) over single-threaded incomplete Cholesky-by-blocks and 19.2x speedup over serial Cholesky performance which does not carry tasking overhead using 56 threads on the Intel Xeon Phi processor for sparse matrices arising from various application problems.

==> abstract.old.tex <==
%% task only

%% PPOPP Guide

%% All submissions must be made electronically through the conference
%% submission site. Abstracts must include contact information, the full
%% list of authors and their affiliations, and a description of the
%% anticipated content of the paper (100-400 words). Full paper
%% submissions must be in PDF formatted for US letter size paper. They
%% must not exceed 10 pages (all inclusive) in standard SIGPLAN
%% two-column conference format (preprint mode, with page numbers).

\begin{abstract}
  We introduce a task-parallel algorithm for sparse
  incomplete Cholesky factorization that utilizes a two dimensional
  sparse partitioned-block layout of a matrix.
  Our factorization algorithm follows the idea of 
  {\it algorithms-by-blocks} by using the block layout. 
  The algorithm-by-blocks approach induces a task graph for the factorization.
  %%which we refine it further for fine-grained parallelism. 
  These tasks are inter-related to each other through their data
  dependences in the factorization algorithm.
  To process the tasks on various manycore architectures in a
  portable manner, we also present a unified tasking API that
  incorporates different tasking backends and device specific
  features using an open-source framework for manycore
  platforms \ie, Kokkos.
  A performance evaluation is presented on both Intel
  Sandybridge and Xeon Phi platforms for matrices from the University
  of Florida sparse matrix collection to illustrate merits of the
  proposed task-based factorization. Experimental results demonstrate
  that our task-parallel implementation delivers about 25X speedup 
  (geometric mean) over sequential performance 
  using 56 threads on the Intel Xeon Phi processor
  for sparse matrices arising from various application problems.
\end{abstract}

  %% We introduce \kj{a task-parallel}{an} algorithm for sparse
  %% incomplete Cholesky factorization that utilizes a two dimensional
  %% sparse\kj{ partitioned}{}-block layout of a matrix.
  %% \kj{Our factorization algorithm follows the idea of 
  %%   {\it algorithms-by-blocks} by using the block layout} 
  %%    {The incomplete factorization is implemented as a
  %%      factorization-by-blocks style algorithm that
  %%      utilizes the block layout}.
  %%    The algorithm-by-blocks approach induces a task graph for the factorization.
  %%    %%which we refine it further for fine-grained parallelism. 
  %%    \kj{These tasks are
  %%   inter-related to each other through their data dependences in the
  %%   factorization algorithm.}{In addition, the incomplete
  %%   factorization is expressed as a set of inter-dependent tasks in a
  %%   task DAG.}
  %% \kj{To process the tasks on various manycore architectures in a
  %%   portable manner, we also present a unified tasking API that
  %%   incorporates different tasking backends and device specific
  %%   features using an open-source framework for manycore
  %%   platforms \ie, Kokkos.}{We also present a tasking API that unifies
  %%   different tasking backends and features of various manycore
  %%   architectures for portable task-based programming.}
  %% \kj{}{The task-based incomplete factorization itself is implemented in a
  %% thread-scalable fashion using the unified task interface of the
  %% Kokkos library.} 
  %% %
  %% \kj{}{The use of the Kokkos high-level abstraction allows our task-based
  %% code to be mapped to various emerging architectures without much
  %% change.} A performance evaluation is presented on both Intel
  %% Sandybridge and Xeon Phi platforms for matrices from the University
  %% of Florida sparse matrix collection to illustrate merits of the
  %% proposed task-based factorization. Experimental results demonstrate
  %% that our task-parallel implementation delivers about 25X speedup 
  %% (geometric mean) over sequential performance 
  %% using 56 threads on the Intel Xeon Phi processor
  %% for sparse matrices arising from various application problems.


%% Old draft
  %% We present an implementation of scalable parallel sparse incomplete
  %% Cholesky factorization using a unified task interface of the Kokkos
  %% library. The parallelism comes from nested dissection that
  %% recursively divides the adjancy graph of a matrix. A
  %% matrix of 2D partitioned blocks based on the tree hierarchy
  %% resulting from the nested dissection is constructed. Next, we apply   
  %% factorization-by-blocks to the matrix of blocks. Tasks are generated
  %% with dependences, which can be expressed by 
  %% a directed acyclic graph for asynchronous parallel execution. 
  %% To dispatch tasks on various emerging hardware architectures, 
  %% Kokkos unified task interface is used. The Kokkos library provides a
  %% performance portable programming model with high-level abstractions
  %% of an execution space and a memory space as well as device-specific
  %% tasking backends. The use of the Kokkos high-level abstraction 
  %% allows our code to be mapped to %%various emerging
  %% architectures without much change.
  %% Numerical experiments are presented for matrices from the
  %% University of Florida sparse matrix collection to illustrate
  %% merits of the proposed task-based factorization.

  %% To illustrate the parallel efficiency of the proposed task-based
  %% factorization, 

  %% In this work, we present numerical experiments of Intel Xeon multi-core
  %% processors and Xeon Phi processors to illustrate the parallel
  %% efficiency of the proposed task-based factorization approach.. 

  %% portable performance and leads a single implementation to be mapped
  %% to various emerging next-generation hardware architectures. 
  %% apply task-parallel sparse factorization to various emerging
  %% hardware architectures,

  %% This feature provides portable performance and
  %% makes a single implementation to be mapped to different
  %% hardware architectures . 
  %% This feature enables our implementation to be efficiently mapped
  %% to various hardware architectures. In this paper,


%% Previous abstract for task-data paper;
%% \begin{abstract}
%%   We present a new strategy for sparse matrix factorization exploiting
%%   both task and data parallelism that can be naturally mapped to
%%   future many-core architecture. In the many-core era, the use of
%%   simd style fine-grained parallelism is necessary to exploit the full
%%   hardware threading capability. The data parallelism can accelerate
%%   the performance of relatively simple matrix-vector multiplication.
%%   However, the sparse matrix factorization is more suitable for using
%%   task paralleism as it can provide many independent tasks using
%%   substructuring techniques \eg, nested dissection. When the sparse
%%   matrix factorization is mapped to the many-core architecture, one
%%   can expect that there exist a performance gap due to the mismatched
%%   characteristics of the irregular application (task-parallel) and
%%   many-core architecture (data-parallel).
%%   We solve this problem by embedding the data parallel model on the
%%   task parallel model. Tasks are spawned following the assembly
%%   tree via standard matrix factorization algorithms; here, we use 
%%   algorithm-by-blocks which views the sparse matrix a collection
%%   blocks. Each task carries a team of threads that matches to the
%%   hardware threading features. For instance, Intel MIC has 4 hardware
%%   threads per computing unit. The spawned tasks are asynchronously
%%   executed after their dependences are satisfied, where each invoked
%%   task exploits data parallelism with its team of threads. Consider
%%   that the tasks generated from sparse matrix factorization is block
%%   matrix factorization, sparse matrix rank-k updates, which is
%%   suitable for using ``parallel for'' (data parallelism).
%%   In this way, we can achieve better locality (as we form a thread team
%%   for a task) and concurrency (as independent tasks are executed
%%   asynchronously). This approach is novel and it has never been
%%   studied in our best knowledge. The proposed approach is implemented
%%   with Qthread for task parallelism and Kokkos for many-core data
%%   paralllsim. 
%% \end{abstract}


==> algorithms/dense-chol.tex <==
\renewcommand{\WSpartitionNarrow}{
  \begin{minipage}[t]{2.0in}
    \begin{tabbing}
      id \= id \= \kill
      {\bf Partition} 
      \partitionings \+ \\
                     {\bf where } 
                     %%%%\begin{minipage}[t]{1.5in}
                     \partitionsizes 
                     %%%%\end{minipage}
    \end{tabbing}
  \end{minipage}
}

\begin{figure*}[h!]
  \begin{center}     % center the algorithm on the page 
    \begin{tabular}{@{\hspace{-0.1in}} p{2.35in} p{2.35in} }

      \resetsteps      % Reset all the commands to create a blank worksheet  

      % Define the operation to be computed

      \renewcommand{\operation}{  A \becomes \mbox{\sc Chol\_unb}( A ) }
      \renewcommand{\routinename}{ A \becomes \mbox{\sc Chol\_unb}( A ) }

      % Step 3: Loop-guard 

      \renewcommand{\guard}{
        length( A_{TL} ) < length( A )
      }

      % Step 8: Insert the updates required to change the 
      %         state from that given in Step 6 to that given in Step 7
      % Note: The below needs editing!!!

      \renewcommand{\update}{
        $ 
        \begin{array}{rcl}
          \alpha_{11} &\becomes& 
          \sqrt{\alpha_{11}} \\
          \tr{a}_{12} &\becomes& 
          \tr{a}_{12}/\alpha_{11} \\
          A_{22} &\becomes& A_{22} - a_{12} \tr{a}_{12} 
        \end{array}
        $
      }

      % Step 4: Redefine Initialize 

      \renewcommand{\partitionings}{
        $
        A \rightarrow
        \FlaTwoByTwo{A_{TL}}{A_{TR}}
                    {A_{BL}}{A_{BR}}
                    $
      }

      \renewcommand{\partitionsizes}{
        $ A_{TL} $ is $ 0 \times 0 $
      }

      % Step 5a: Repartition the operands 

      \renewcommand{\blocksize}{blank}
      \renewcommand{\repartitionings}{
        $
        \FlaTwoByTwo{\color{red}A_{TL}}{\color{blue}A_{TR}}
                    {\color{cyan}A_{BL}}{A_{BR}}
                    %$ \\
                    %~~~~ 
                    %$  
                    \rightarrow
                    \FlaThreeByThreeBR{\color{red}A_{00}}{\color{blue}a_{01}}{\color{blue}A_{02}}
                                      {\color{cyan}\tr{a}_{10}}{\alpha_{11}}{ \tr{a}_{12} }
                                      {\color{cyan}A_{20}}{a_{21}}{A_{22}}
                                      $}

      \renewcommand{\repartitionsizes}{
        $ \alpha_{11} $ is a scalar
      }

      % Step 5b: Move the double lines 

      \renewcommand{\moveboundaries}{
        $
        \FlaTwoByTwo{\color{red}A_{TL}}{\color{blue}A_{TR}}
                    {\color{cyan}A_{BL}}{A_{BR}}
                    %$ \\
                    %~~~~ 
                    %$  
                    \leftarrow
                    \FlaThreeByThreeTL{\color{red}A_{00}}{\color{red}a_{01}}{\color{blue}A_{02}}
                                      {\color{red}\tr{a}_{10}}{\color{red}\alpha_{11}}{\color{blue}\tr{a}_{12}}
                                      {\color{cyan}A_{20}}{\color{cyan}a_{21}}{A_{22}}
                                      $}
      \begin{minipage}[t]{2.35in} 
        \setlength{\arraycolsep}{2pt}
        \footnotesize 
        \FlaAlgorithmNarrow
        % this command generates the algorithm 
      \end{minipage}
      &
      \resetsteps      % Reset all the commands to create a blank worksheet  

      % Define the operation to be computed

      \renewcommand{\operation}{  A \becomes \mbox{\sc Chol\_blk}( A ) }
      \renewcommand{\routinename}{ A \becomes \mbox{\sc Chol\_blk}( A ) }

      % Step 3: Loop-guard 

      \renewcommand{\guard}{
        length( A_{TL} ) < length( A )
      }

      % Step 8: Insert the updates required to change the 
      %         state from that given in Step 6 to that given in Step 7
      % Note: The below needs editing!!!

      \renewcommand{\update}{
        $ 
        \begin{array}{rcl}
    A_{11} &\becomes& \mbox{\sc Chol\_unb}( A_{11} )  \\
    A_{12} &\becomes& \triu{A_{11}}^{-1} A_{12}   \\
    A_{22} &\becomes& A_{22} - \tr{A}_{12} A_{12}   
        \end{array}
        $
      }

      % Step 4: Redefine Initialize 

      \renewcommand{\partitionings}{
        $
        A \rightarrow
        \FlaTwoByTwo{A_{TL}}{A_{TR}}
                    {A_{BL}}{A_{BR}}
                    $
      }

      \renewcommand{\partitionsizes}{
        $ A_{TL} $ is $ 0 \times 0 $
      }

      % Step 5a: Repartition the operands 

      \renewcommand{\blocksize}{b}
      \renewcommand{\repartitionings}{
        $
        \FlaTwoByTwo{\color{red}A_{TL}}{\color{blue}A_{TR}}
                    {\color{cyan}A_{BL}}{A_{BR}}
                    %$ \\
                    %~~~~ 
                    %$  
                    \rightarrow
                    \FlaThreeByThreeBR{\color{red}A_{00}}{\color{blue}A_{01}}{\color{blue}A_{02}}
                                      {\color{cyan}A_{10}}{A_{11}}{A_{12} }
                                      {\color{cyan}A_{20}}{A_{21}}{A_{22}}
                                      $}

      \renewcommand{\repartitionsizes}{
        $ A_{11} $ is $ \blocksize \times \blocksize $
      }

      % Step 5b: Move the double lines 

      \renewcommand{\moveboundaries}{
        $
        \FlaTwoByTwo{\color{red}A_{TL}}{\color{blue}A_{TR}}
                    {\color{cyan}A_{BL}}{A_{BR}}
                    %$ \\
                    %~~~~ 
                    %$  
                    \leftarrow
                    \FlaThreeByThreeTL{\color{red}A_{00}}{\color{red}A_{01}}{\color{blue}A_{02}}
                                      {\color{red}A_{10}}{\color{red}A_{11}}{\color{blue}A_{12} }
                                      {\color{cyan}A_{20}}{\color{cyan}A_{21}}{A_{22}}
                                      $}
      \begin{minipage}[t]{2.35in} 
        \setlength{\arraycolsep}{2pt}
        \footnotesize 
        \FlaAlgorithmNarrow
        % this command generates the algorithm 
      \end{minipage}
    \end{tabular}
  \end{center} 
  
  % The following command creates a caption for the figure. 
  
  \caption{Cholesky factorization algorithms.}
  \label{fig:dense-chol}
\end{figure*}%[p]



==> algorithms/sparse-chol-by-blocks-detail.tex <==

\renewcommand{\FlaStartComputeShorter}{
  \setlength{\unitlength}{0.5in}
  \begin{picture}(5.5,0.01)
    \put(0,0){\line(1,0){5.5}}
    \put(0,0.01){\line(1,0){5.5}}
  \end{picture}
}  
\renewcommand{\FlaEndComputeShorter}{
  \setlength{\unitlength}{0.5in}
  \begin{picture}(5.5,0.01)
    \put(0,0){\line(1,0){5.5}}
    \put(0,0.01){\line(1,0){5.5}}
  \end{picture}
}  

\begin{figure}[tb!]
  \begin{center}     % center the algorithm on the page 
      \resetsteps      % Reset all the commands to create a blank worksheet  

      % Define the operation to be computed

      \renewcommand{\operation}{  A \becomes \mbox{\sc Chol\_by\_blocks}( A ) }
      \renewcommand{\routinename}{ A \becomes \mbox{\sc Chol\_by\_blocks}( A ) }

      % Step 3: Loop-guard 

      \renewcommand{\guard}{
        length( A_{TL} ) < length( A )
      }

      % Step 8: Insert the updates required to change the 
      %         state from that given in Step 6 to that given in Step 7
      % Note: The below needs editing!!!
      
      \renewcommand{\update}{
      }

      % Step 4: Redefine Initialize 

      \renewcommand{\partitionings}{
        $
        A \rightarrow
        \FlaTwoByTwo{A_{TL}}{A_{TR}}
                    {A_{BL}}{A_{BR}}
                    $
      }

      \renewcommand{\partitionsizes}{
        $ A_{TL} $ is $ 0 \times 0 $
      }

      % Step 5a: Repartition the operands 

      \renewcommand{\blocksize}{1}
      \renewcommand{\repartitionings}{
        $
        \FlaTwoByTwo{\color{red}A_{TL}}{\color{blue}A_{TR}}
                    {\color{cyan}A_{BL}}{A_{BR}}
                    %$ \\
                    %~~~~ 
                    %$  
                    \rightarrow
                    \FlaThreeByThreeBR{\color{red}A_{00}}{\color{blue}A_{01}}{\color{blue}A_{02}}
                                      {\color{cyan}A_{10}}{A_{11}}{A_{12} }
                                      {\color{cyan}A_{20}}{A_{21}}{A_{22}}
                                      $}

      \renewcommand{\repartitionsizes}{
        $ A_{11} $ is $ \blocksize \times \blocksize $
      }

      % Step 5b: Move the double lines 

      \renewcommand{\moveboundaries}{
        $
        \FlaTwoByTwo{\color{red}A_{TL}}{\color{blue}A_{TR}}
                    {\color{cyan}A_{BL}}{A_{BR}}
                    %$ \\
                    %~~~~ 
                    %$  
                    \leftarrow
                    \FlaThreeByThreeTL{\color{red}A_{00}}{\color{red}A_{01}}{\color{blue}A_{02}}
                                      {\color{red}A_{10}}{\color{red}A_{11}}{\color{blue}A_{12} }
                                      {\color{cyan}A_{20}}{\color{cyan}A_{21}}{A_{22}}
                                      $}
      \begin{minipage}[t]{3.2in} 
        \setlength{\arraycolsep}{2pt}
        \footnotesize 
        \begin{center}
          \begin{tabular}{|l |} \hline
            {\bf Algorithm:} $\routinename$ \\ \whline
            {\WSpartitionNarrow} \\
            {\bf while} \WSguard { \bf do} \\
            \ \hspace{0.0in} \WSrepartitionNarrow \\
            {\hspace{0.0in} \FlaStartComputeShorter} \\
            {\hspace{0.0in}
              \begin{array}{rclcr}
                A_{11} &\becomes& \mbox{\sc Chol}( A_{11} ) & \qquad
                & \mbox{\tt genTaskChol}  \\
                A_{12} &\becomes& \triu{A_{11}}^{-1} A_{12} & \qquad
                & \mbox{\tt genTaskTrsm} \\
                A_{22} &\becomes& A_{22} - \tr{A}_{12}A_{12} & \qquad
                & \mbox{\tt genTaskHerk} 
              \end{array}  
            } \\
            {\hspace{0.0in} \FlaEndComputeShorter} \\
            {\ \hspace{0.0in} \WSmoveboundaryNarrow} \\
            {{\bf endwhile}} \\ \hline
          \end{tabular}
        \end{center} 
        %\FlaAlgorithmNarrow
        % this command generates the algorithm 
      \end{minipage}
  \end{center} 
  \vspace{\figup}
  % The following command creates a caption for the figure. 
  
  \caption{Cholesky-by-blocks algorithm on a 2D partitioned-block
    matrix. The blocks in the $2\times2$
    and $3\times3$ block matrices that correspond to each other are of 
    the same color.}
  \label{fig:sparse-chol}
\end{figure}%[p]



==> codes/crs_matrix_base.tex <==
\begin{code}[tb!]
  \lstsetbylang{C++}
  \begin{center}
    \begin{lstlisting}[mathescape]
template<typename value_type,
         typename ordinal_type,
         typename size_type>
class CrsMatrixBase {
public:           
  // Kokkos view array
  typedef Kokkos::View<size_type*>    size_type_array;
  typedef Kokkos::View<ordinal_type*> ordinal_type_array;
  typedef Kokkos::View<value_type*>   value_type_array;

private:                                                                                                  
  ordinal_type       _m;       // # of rows
  ordinal_type       _n;       // # of cols
  size_type          _nnz;     // # of nonzeros

  size_type_array    _ap;      // pointers to row index
  ordinal_type_array _aj;      // column index array
  value_type_array   _ax;      // value array 
};
    \end{lstlisting}
  \end{center}
  \caption{CrsMatrixBase; a flat matrix has a value type as a scalar
    object while a hierarchically partitioned matrix has a value type
    as a matrix view object.}
  \label{code:crs_matrix_base}
\end{code}


==> codes/crs_matrix_view.tex <==
\begin{code}[tb!]
  \lstsetbylang{C++}
  \begin{center}
    \begin{lstlisting}[mathescape]
template<typename CrsMatixBaseType>
class CrsMatrixView {
private:
  // a pointer to the base matrix  
  CrsMatrixBaseType *_base;         

  // offsets and dimension in row and column
  ordinal_type       _offm, _offn;  
  ordinal_type       _m, _n;        

public:
  // columns of a row associated with this view
  CrsRowView RowView(const ordinal_type i) const; 
};

template<typename CrsMatrixViewType>
class CrsTaskView : public CrsMatrixViewType {
public:
  typedef Kokkos::TaskPolicy  policy_type;
  typedef Kokkos::Future<int> future_type;

private:
  // handle for tasks associated with this view 
  future_type _future;

public:
  void setFuture(const future_type &f);  
  future_type Future() const;            
};
    \end{lstlisting}
  \end{center}
  \caption{A view object indicates a rectangular region
    of the base matrix set by its offset and dimension values.}
  \label{code:crs_matrix_view}
\end{code}


==> codes/ichol_by_blocks.tex <==
\begin{code}[tb!]
  \lstsetbylang{C++}
  \begin{center}
    \begin{lstlisting}[mathescape]
class ICholByBlocks<Uplo::Upper> {
public:
  typedef Kokkos::TaskPolicy policy_type;

  // Kokkos tasking interface functor
  class TaskFunctor {
    void apply(value_type &r_val) {
      CrsTaskView ATL, ATR,     A00, A01, A02,
                  ABL, ABR,     A10, A11, A12,
                                A20, A21, A22;

      Part_2x2(A,  ATL, ATR,
                   ABL, ABR,
               0, 0, Partition::TopLeft);

      while (ATL.NumRows() < A.NumRows()) {
        Part_2x2_to_3x3(ATL,/**/ ATR, A00,/**/ A01, A02,
                        /***********//*****************/
                                      A10,/**/ A11, A12,
                        ABL,/**/ ABR, A20,/**/ A21, A22,
                        1, 1, Partition::BottomRight);
        // ---------------------------------------------
        genICholTask(policy, A11);     
        genTrsmTasks(policy, A11, A12); 
        genHerkTasks(policy, A12, A22); 
        // ---------------------------------------------
        Merge_3x3_to_2x2(A00, A01,/**/ A02, ATL,/**/ ATR,
                         A10, A11,/**/ A12,
                         /****************//************/
                         A20, A21,/**/ A22, ABL,/**/ ABR,
                         Partition::TopLeft);
      }
    }
  };
};
    \end{lstlisting}
  \end{center}
  \caption{Cholesky-by-blocks on a 2D partitioned-block matrix.}
  \label{code:ichol_by_blocks}
\end{code}


==> codes/ichol_by_blocks_detail.tex <==
%% \begin{code}[tb!]
%%   \lstsetbylang{C++}
%%   \begin{center}
%%     \begin{lstlisting}[mathescape]
%% void ICholByBlocks<Uplo::Upper>::TaskFunctor
%% ::genICHolTask(policy_type &policy, CrsTaskViewType &A) {
%%   // get a block A(0,0)
%%   value_type aa = A.RowView(0).Value(0);

%%   // construct a task
%%   future_type f = policy.create(IChol<Uplo::Upper>
%%                                 ::TaskFunctor<value_type>(aa));

%%   // manage dependence
%%   policy.add_dependence(f, aa.Future());
%%   aa.setFuture(f);

%%   // spawn the task
%%   policy.spawn(f);    
%% }
%%     \end{lstlisting}
%%   \end{center}
%%   \caption{Task spawning in ICholByBlocks: \mbox{\sc Chol} task.}
%%   \label{code:ichol_by_blocks:scalar}
%% \end{code}

\begin{code}[tb!]
  \lstsetbylang{C++}
  \begin{center}
    \begin{lstlisting}[mathescape]
void ICholByBlocks<Uplo::Upper>::TaskFunctor
::genTrsmTask(policy_type &policy,
              CrsTaskViewType &A,
              CrsTaskViewType &B) {
  // get a block A(0,0) and row view of B(0,:)
  value_type &aa = A.RowView(0).Value(0);
  row_view_type b = B.RowView(0);

  // update the row b
  for (ordinal_type j=0;j<b.NumNonZeros();++j) {
    value_type bb = b.Value(j);

    // construct a task
    future_type f = policy.create(
         Trsm<Side::Left,Uplo::Upper,Trans::ConjTranspose>
         ::TaskFunctor(Diag::NonUnit, 1.0, aa, bb));

    // manage dependence
    policy.add_dependence(f, aa.Future());
    policy.add_dependence(f, bb.Future());
    bb.setFuture(f);

    // spawn the task
    policy.spawn(f);
  }
}
    \end{lstlisting}
  \end{center}
  \caption{Task spawning in \texttt{genTrsmTasks}.}
  \label{code:ichol_by_blocks:trsm}
\end{code}



%% \begin{code}[tb!]
%%   \lstsetbylang{C++}
%%   \begin{center}
%%     \begin{lstlisting}[mathescape]
%% void ICholByBlocks<Uplo::Upper>::TaskFunctor<CrsTaskViewType>
%% ::genHerkTask(policy_type &policy, CrsTaskViewType &A, CrsTaskViewType &C) {
%%   // get a row A(0,:) and row view of C(0)
%%   row_view_type a = A.RowView(0);
%%   row_view_type c = C.RowView(0);

%%   // loop over a row a
%%   for (ordinal_type i=0;i<a.NumNonZeros();++i) {  
%%     value_type aa = a.Value(i);

%%     const ordinal_type row_at_i = a.Col(i);
%%     row_view_type c = C.RowView(row_at_i);

%%     // loop over a^T
%%     ordinal_type idx = 0;
%%     for (ordinal_type j=i;j<a.NumNonZeros() && idx != End;++j) {
%%       value_type bb = a.Value(j);
%%       const ordinal_type col_at_j = a.Col(j);

%%       // find an index of the updating block
%%       idx = c.Index(col_at_j);
%%       if (idx != End) {
%%         const bool is_diagonal = (row_at_i == col_at_j);
%%         value_type cc = c.Value(idx);

%%         // for a diagonal block, create a Herk task; otherwise, create a Gemm task
%%         future_type f = policy.create(is_diagonal ?
%%                                       Herk<Uplo::Upper,Trans::ConjTranspose>
%%                                       ::TaskFunctor<value_type>(-1.0, aa, 1.0, cc) :
%%                                       Gemm<Trans::ConjTranspose,Trans::NoTranspose>::
%%                                       ::TaskFunctor<value_type>(-1.0, aa, bb, 1.0, cc));

%%         // manage dependence
%%         policy.add_dependence(f, aa.Future());
%%         if (!is_diagonal)
%%           policy.add_dependence(f, bb.Future());
%%         policy.add_dependence(f, cc.Future());
%%         cc.setFuture(f);

%%         // spawn the task
%%         policy.spawn(f);
%%       }
%%     }
%%   }
%% }
%%     \end{lstlisting}
%%   \end{center}
%%   \caption{Task spawning in ICholByBlocks: \mbox{\sc Herk} task.}
%%   \label{code:ichol_by_blocks:herk}
%% \end{code}



==> codes/ichol_by_blocks_driver.tex <==
\begin{code}[tb!]
  \lstsetbylang{C++}
  \begin{center}
    \begin{lstlisting}[mathescape]
void driver() {
  typedef int          ordinal_type;
  typedef unsigned int size_type;
  typedef double       value_type;
  
  typedef CrsMatrixBase<value_type,ordinal_type,size_type> CrsMatrixBaseType; 
  typedef TaskView<CrsMatrixView<CrsMatrixBaseType> > CrsTaskViewType; 
  
  typedef CrsMatrixBase<CrsTaskViewType,ordinal_type,size_type> CrsHierMatrixBaseType;
  typedef TaskView<CrsHierMatrixView<CrsHierMatrixBaseType> CrsHierTaskViewType;
  
  CraMatrixBaseType A(``Input SPD Matrix'');
  A.importMatrix(``filename.mtx'');
  
  CrsMatrixBaseType U(``Upper Factors'');
  GraphHelper S(A);
  S.computeOrdering();
  
  U.copy(Uplo::Upper, A, S.PermVector(), S.InvPermVector());
  
  CrsHierMatrixBaseType H(``Hier Matrix'');
  flat2hier(Uplo::Upper, U, H, S.NumBlocks(), S.RangeVector(), S.TreeVector());
  
  Kokkos::TaskPolicy policy;
  auto future = policy.create(ICholByBlocks<Uplo::Upper>::TaskFunctor<matrix_view_type>(H);
  policy.spawn(future);
  Kokkos::wait(policy);
}
    \end{lstlisting}
  \end{center}
  \caption{Example driver code for task-based incomplete Cholesky-by-blocks.}
  \label{code:ichol_by_blocks:driver}
\end{code}


==> codes/ichol_symbolic.tex <==
\begin{code}[tb!]
  \lstsetbylang{C++}
  \begin{center}
    \begin{lstlisting}[mathescape]

template<typename CrsMatrixType>      
class SymbolicFactor {
  CrsMatrixType _A;
  
  class FunctorComputeNonZeroPatternInRow {
    public:
    typedef Kokkos::TeamPolicy policy_type;  // task execution policy
    
    // league specific work space object type
    Kokkos::View<ordinal_type**, Kokkos::LayoutLeft> league_specific_ordinal_type_array;
    
    private:
    ordinal_type _level;
    ordinal_type _ml
    crs_graph_type _graph;
    
    league_specific_ordinal_type_array _queue;
    league_specific_ordinal_type_array _visited;
    league_specific_ordinal_type_array _distance;
    
    public:
    KOKKOS_INLINE_FUNCTION  
    void operator()(const typename policy_type::member_type &member) const {       
      // membership in the league
      const int lrank = member.league_rank();
      const int lsize = member.league_size();
      
      // league workspace
      league_specific_ordinal_type_array_ptr queue    = &_queue(0, lrank);
      league_specific_ordinal_type_array_ptr distance = &_distance(0, lrank);
      league_specific_ordinal_type_array_ptr visited  = &_visited(0, lrank);  
      
      for (ordinal_type i=lrank;i<_m;i+=lsize) {
        Queue q(queue);
        
        q.push(i);
        distance[i] = 0;
        
        const ordinal_type id = (i+1);
        visited[i] = id;
        
        while (!q.empty()) {
          const ordinal_type h = q.pop();
          
          const ordinal_type jbegin = _graph._ap[h], jend = _graph._ap[h+1];
          for (ordinal_type j=jbegin;j<jend;++j) {
            const ordinal_type t = _graph._aj[j];
            if (visited[t] != id) {
              visited[t] = id;
              
              if (t < i && distance[h] < _level) {
                q.push(t);
                distance[t] = distance[h] + 1;
              }
              if (t > i) 
              _aj[cnt++] = t;
            }
          }
        }
        
        q.clear();
      }
    }
  };

  void createNonZeroPattern(const ordinal_type level) {
    FunctorComputeNonZeroPatternInRow functor(level);
    Kokkos::parallel_for(typename FunctorComputeNonZeroPatternInRow::policy_type(_lsize, 1), functor);
  }
  
};
    \end{lstlisting}
  \end{center}
  \caption{Cholesky-by-blocks on a hierarchically partitioned matrix.}
  \label{code:ichol_by_blocks}
\end{code}



==> keyword.tex <==
\keywords{%
  Directed Acyclic Graph, Cholesky, Many-core, Task parallelism, Data
  parallelism, Kokkos, Qthreads, Algorithm-by-blocks
}

